Domain Generalisation for Object Detection under Covariate and Concept Shift

Domain generalisation aims to promote the learning of domain-invariant features while suppressing domain-specific features, so that a model can generalise better to previously unseen target domains. An approach to domain generalisation for object detection is proposed, the first such approach applicable to any object detection architecture. Based on a rigorous mathematical analysis, we extend approaches based on feature alignment with a novel component for performing class conditional alignment at the instance level, in addition to aligning the marginal feature distributions across domains at the image level. This allows us to fully address both components of domain shift, i.e. covariate and concept shift, and learn a domain agnostic feature representation. We perform extensive evaluation with both one-stage (FCOS, YOLO) and two-stage (FRCNN) detectors, on a newly proposed benchmark comprising several different datasets for autonomous driving applications (Cityscapes, BDD10K, ACDC, IDD) as well as the GWHD dataset for precision agriculture, and show consistent improvements to the generalisation and localisation performance over baselines and state-of-the-art.

==> references_backup.tex <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})

@inproceedings{idd-dataset,
  title={IDD: A dataset for exploring problems of autonomous navigation in unconstrained environments},
  author={G.~Varma and A.~Subramanian and A.~Namboodiri and M.~Chandraker and C.~V.~Jawahar},
  booktitle={2019 IEEE Winter Conference on Applications of Computer Vision (WACV)},
  pages={1743--1751},
  year={2019}
}

@InProceedings{acdc-dataset,
  author = {Sakaridis, Christos and Dai, Dengxin and Van Gool, Luc},
  title = {{ACDC}: The Adverse Conditions Dataset with Correspondences for Semantic Driving Scene Understanding},
  booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
  month = {October},
  year = 2021
}

@article{wu2021instance,
  title={Instance-Invariant Domain Adaptive Object Detection via Progressive Disentanglement},
  author={Wu, Aming and Han, Yahong and Zhu, Linchao and Yang, Yi},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2021},
  publisher={IEEE}
}

@article{endres2003new,
  title={A new metric for probability distributions},
  author={Endres, Dominik Maria and Schindelin, Johannes E},
  journal={IEEE Transactions on Information theory},
  volume={49},
  number={7},
  pages={1858--1860},
  year={2003},
  publisher={IEEE}
}

@article{scholkopf2012causal,
  title={On causal and anticausal learning},
  author={Sch{\"o}lkopf, Bernhard and Janzing, Dominik and Peters, Jonas and Sgouritsa, Eleni and Zhang, Kun and Mooij, Joris},
  journal={arXiv preprint arXiv:1206.6471},
  year={2012}
}

@article{janzing2010causal,
  title={Causal inference using the algorithmic Markov condition},
  author={Janzing, Dominik and Sch{\"o}lkopf, Bernhard},
  journal={IEEE Transactions on Information Theory},
  volume={56},
  number={10},
  pages={5168--5194},
  year={2010},
  publisher={IEEE}
}


@inproceedings{matsuura2020domain,
  title={Domain generalization using a mixture of multiple latent domains},
  author={Matsuura, Toshihiko and Harada, Tatsuya},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={34},
  pages={11749--11756},
  year={2020}
}

@article{ren2015faster,
  title={Faster {R-CNN}: Towards real-time object detection with region proposal networks},
  author={Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
  journal={Advances in neural information processing systems},
  volume={28},
  pages={91--99},
  year={2015}
}

@inproceedings{koh2021wilds,
  title={Wilds: A benchmark of in-the-wild distribution shifts},
  author={Koh, Pang Wei and Sagawa, Shiori and Xie, Sang Michael and Zhang, Marvin and Balsubramani, Akshay and Hu, Weihua and Yasunaga, Michihiro and Phillips, Richard Lanas and Gao, Irena and Lee, Tony and others},
  booktitle={International Conference on Machine Learning},
  pages={5637--5664},
  year={2021},
  organization={PMLR}
}

@inproceedings{khirodkar2019domain,
  title={Domain randomization for scene-specific car detection and pose estimation},
  author={Khirodkar, Rawal and Yoo, Donghyun and Kitani, Kris},
  booktitle={2019 IEEE Winter Conference on Applications of Computer Vision (WACV)},
  pages={1932--1940},
  year={2019},
  organization={IEEE}
}

@article{david2021global,
  title={Global Wheat Head Detection 2021: an improved dataset for benchmarking wheat head detection methods},
  author={David, Etienne and Serouart, Mario and Smith, Daniel and Madec, Simon and Velumani, Kaaviya and Liu, Shouyang and Wang, Xu and Pinto, Francisco and Shafiee, Shahameh and Tahir, Izzat SA and others},
  journal={Plant Phenomics},
  volume={2021},
  year={2021},
  publisher={AAAS}
}

@article{david2020global,
  title={Global Wheat Challenge 2020: Analysis of the competition design and winning models},
  author={David, Etienne and Ogidi, Franklin and Guo, Wei and Baret, Frederic and Stavness, Ian},
  journal={arXiv preprint arXiv:2105.06182},
  year={2021}
}

@article{moreno2012unifying,
  title={A unifying view on dataset shift in classification},
  author={Moreno-Torres, Jose G and Raeder, Troy and Alaiz-Rodr{\'\i}guez, Roc{\'\i}o and Chawla, Nitesh V and Herrera, Francisco},
  journal={Pattern recognition},
  volume={45},
  number={1},
  pages={521--530},
  year={2012},
  publisher={Elsevier}
}


@article{zhuang2020comprehensive,
  title={A comprehensive survey on transfer learning},
  author={Zhuang, Fuzhen and Qi, Zhiyuan and Duan, Keyu and Xi, Dongbo and Zhu, Yongchun and Zhu, Hengshu and Xiong, Hui and He, Qing},
  journal={Proceedings of the IEEE},
  volume={109},
  number={1},
  pages={43--76},
  year={2020}
}

@article{niu2020decade,
  title={A decade survey of transfer learning (2010--2020)},
  author={Niu, Shuteng and Liu, Yongxin and Wang, Jian and Song, Houbing},
  journal={IEEE Transactions on Artificial Intelligence},
  volume={1},
  number={2},
  pages={151--166},
  year={2020}
}

@inproceedings{fang2013unbiased,
  title={Unbiased metric learning: On the utilization of multiple datasets and web images for softening bias},
  author={Fang, Chen and Xu, Ye and Rockmore, Daniel N},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={1657--1664},
  year={2013}
}

@article{ghazi2017plant,
  title={Plant identification using deep neural networks via optimization of transfer learning parameters},
  author={Ghazi, Mostafa Mehdipour and Yanikoglu, Berrin and Aptoula, Erchan},
  journal={Neurocomputing},
  volume={235},
  pages={228--235},
  year={2017}
}

@inproceedings{saenko2010adapting,
  title={Adapting visual category models to new domains},
  author={Saenko, Kate and Kulis, Brian and Fritz, Mario and Darrell, Trevor},
  booktitle={European Conference on Computer Vision},
  pages={213--226},
  year={2010},
  organization={Springer}
}

@inproceedings{torralba2011unbiased,
  title={Unbiased look at dataset bias},
  author={Torralba, Antonio and Efros, Alexei A},
  booktitle={CVPR 2011},
  pages={1521--1528},
  year={2011},
  organization={IEEE}
}

@inproceedings{khosla2012undoing,
  title={Undoing the damage of dataset bias},
  author={Khosla, Aditya and Zhou, Tinghui and Malisiewicz, Tomasz and Efros, Alexei A and Torralba, Antonio},
  booktitle={European Conference on Computer Vision},
  pages={158--171},
  year={2012},
  organization={Springer}
}

@inproceedings{xu2014exploiting,
  title={Exploiting low-rank structure from latent domains for domain generalization},
  author={Xu, Zheng and Li, Wen and Niu, Li and Xu, Dong},
  booktitle={European Conference on Computer Vision},
  pages={628--643},
  year={2014},
  organization={Springer}
}

@inproceedings{li2018learning,
  title={Learning to generalize: Meta-learning for domain generalization},
  author={Li, Da and Yang, Yongxin and Song, Yi-Zhe and Hospedales, Timothy M},
  booktitle={Thirty-Second AAAI Conference on Artificial Intelligence},
  year={2018}
}

@inproceedings{shankar2018generalizing,
  title={Generalizing across domains via cross-gradient training},
  author={Shankar, Shiv and Piratla, Vihari and Chakrabarti, Soumen and Chaudhuri, Siddhartha and Jyothi, Preethi and Sarawagi, Sunita},
  booktitle={ICLR},
  year={2018}
}

@inproceedings{tobin2017domain,
  title={Domain randomization for transferring deep neural networks from simulation to the real world},
  author={Tobin, Josh and Fong, Rachel and Ray, Alex and Schneider, Jonas and Zaremba, Wojciech and Abbeel, Pieter},
  booktitle={2017 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={23--30},
  year={2017},
  organization={IEEE}
}

@inproceedings{song2019generalizable,
  title={Generalizable person re-identification by domain-invariant mapping network},
  author={Song, Jifei and Yang, Yongxin and Song, Yi-Zhe and Xiang, Tao and Hospedales, Timothy M},
  booktitle={Proceedings of the IEEE/CVF conference on Computer Vision and Pattern Recognition},
  pages={719--728},
  year={2019}
}

@inproceedings{wang2020cross,
  title={Cross-domain face presentation attack detection via multi-domain disentangled representation learning},
  author={Wang, Guoqing and Han, Hu and Shan, Shiguang and Chen, Xilin},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={6678--6687},
  year={2020}
}

@inproceedings{jia2020single,
  title={Single-side domain generalization for face anti-spoofing},
  author={Jia, Yunpei and Zhang, Jie and Shan, Shiguang and Chen, Xilin},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8484--8493},
  year={2020}
}


@inproceedings{li2017deeper,
  title={Deeper, broader and artier domain generalization},
  author={Li, Da and Yang, Yongxin and Song, Yi-Zhe and Hospedales, Timothy M},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={5542--5550},
  year={2017}
}

@inproceedings{ghifary2015domain,
  title={Domain generalization for object recognition with multi-task autoencoders},
  author={Ghifary, Muhammad and Kleijn, W Bastiaan and Zhang, Mengjie and Balduzzi, David},
  booktitle={Proceedings of the IEEE International Conference on Vision},
  pages={2551--2559},
  year={2015}
}

@inproceedings{gong2019dlow,
  title={Dlow: Domain flow for adaptation and generalization},
  author={Gong, Rui and Li, Wen and Chen, Yuhua and Gool, Luc Van},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2477--2486},
  year={2019}
}

@article{dou2019domain,
  title={Domain generalization via model-agnostic learning of semantic features},
  author={Dou, Qi and Coelho de Castro, Daniel and Kamnitsas, Konstantinos and Glocker, Ben},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@inproceedings{du2020metanorm,
  title={Metanorm: Learning to normalize few-shot batches across domains},
  author={Du, Yingjun and Zhen, Xiantong and Shao, Ling and Snoek, Cees GM},
  booktitle={International Conference on Learning Representations},
  year={2020}
}


@inproceedings{finn2017model,
  title={Model-agnostic meta-learning for fast adaptation of deep networks},
  author={Finn, Chelsea and Abbeel, Pieter and Levine, Sergey},
  booktitle={International conference on machine learning},
  pages={1126--1135},
  year={2017},
  organization={PMLR}
}

@inproceedings{shi2022gradient,
title={Gradient Matching for Domain Generalization},
author={Yuge Shi and Jeffrey Seely and Philip Torr and Siddharth N and Awni Hannun and Nicolas Usunier and Gabriel Synnaeve},
booktitle={International Conference on Learning Representations},
year={2022},
url={https://openreview.net/forum?id=vDwBW49HmO}
}

@inproceedings{ilse2020diva,
  title={Diva: Domain invariant variational autoencoders},
  author={Ilse, Maximilian and Tomczak, Jakub M and Louizos, Christos and Welling, Max},
  booktitle={Medical Imaging with Deep Learning},
  pages={322--348},
  year={2020},
  organization={PMLR}
}


@article{volpi2018generalizing,
  title={Generalizing to unseen domains via adversarial data augmentation},
  author={Volpi, Riccardo and Namkoong, Hongseok and Sener, Ozan and Duchi, John and Murino, Vittorio and Savarese, Silvio},
  journal={arXiv preprint arXiv:1805.12018},
  year={2018}
}

@inproceedings{gan2016learning,
  title={Learning attributes equals multi-source domain generalization},
  author={Gan, Chuang and Yang, Tianbao and Gong, Boqing},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={87--97},
  year={2016}
}

@inproceedings{muandet2013domain,
  title={Domain generalization via invariant feature representation},
  author={Muandet, Krikamol and Balduzzi, David and Sch{\"o}lkopf, Bernhard},
  booktitle={International Conference on Machine Learning},
  pages={10--18},
  year={2013},
  organization={PMLR}
}

@inproceedings{cordts2016cityscapes,
  title={The {C}ityscapes dataset for semantic urban scene understanding},
  author={Cordts, Marius and Omran, Mohamed and Ramos, Sebastian and Rehfeld, Timo and Enzweiler, Markus and Benenson, Rodrigo and Franke, Uwe and Roth, Stefan and Schiele, Bernt},
  booktitle={Proceedings of the IEEE Conference on Computer Cision and Pattern Recognition},
  pages={3213--3223},
  year={2016}
}




@article{cai2021uncertainty,
  title={Uncertainty-Aware Model Adaptation for Unsupervised Cross-Domain Object Detection},
  author={Cai, Minjie and Luo, Minyi and Zhong, Xionghu and Chen, Hao},
  journal={arXiv preprint arXiv:2108.12612},
  year={2021}
}

@inproceedings{li2018deep,
  title={Deep domain generalization via conditional invariant adversarial networks},
  author={Li, Ya and Tian, Xinmei and Gong, Mingming and Liu, Yajing and Liu, Tongliang and Zhang, Kun and Tao, Dacheng},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={624--639},
  year={2018}
}

@INPROCEEDINGS{10204463,
  author={Zhang, Gongjie and Luo, Zhipeng and Tian, Zichen and Zhang, Jingyi and Zhang, Xiaoqin and Lu, Shijian},
  booktitle={2023 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={Towards Efficient Use of Multi-Scale Features in Transformer-Based Object Detectors}, 
  year={2023},
  pages={6206--6216}
}

@INPROCEEDINGS{10204055,
  author={Huang, Zhou and Dai, Hang and Xiang, Tian-Zhu and Wang, Shuo and Chen, Huai-Xin and Qin, Jie and Xiong, Huan},
  booktitle={2023 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={Feature Shrinkage Pyramid for Camouflaged Object Detection with Transformers}, 
  year={2023},
  pages={5557--5566}
}

@InProceedings{He2022CVPR,
    author    = {He, Liqiang and Todorovic, Sinisa},
    title     = {DESTR: Object Detection With Split Transformer},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2022},
    pages     = {9377-9386}
}

@inproceedings{carion2020end,
  title={End-to-end object detection with transformers},
  author={Carion, Nicolas and Massa, Francisco and Synnaeve, Gabriel and Usunier, Nicolas and Kirillov, Alexander and Zagoruyko, Sergey},
  booktitle={European conference on computer vision},
  pages={213--229},
  year={2020},
  organization={Springer}
}

@inproceedings{chen2018domain,
  title={Domain adaptive {F}aster {R-CNN} for object detection in the wild},
  author={Chen, Yuhua and Li, Wen and Sakaridis, Christos and Dai, Dengxin and Van Gool, Luc},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3339--3348},
  year={2018}
}

@article{gong2019twin,
  title={Twin auxiliary classifiers {GAN}},
  author={Gong, Mingming and Xu, Yanwu and Li, Chunyuan and Zhang, Kun and Batmanghelich, Kayhan},
  journal={Advances in neural information processing systems},
  volume={32},
  pages={1328},
  year={2019},
  publisher={NIH Public Access}
}

@article{zhao2020domain,
  title={Domain generalization via entropy regularization},
  author={Zhao, Shanshan and Gong, Mingming and Liu, Tongliang and Fu, Huan and Tao, Dacheng},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  year={2020}
}

@inproceedings{li2018domain,
  title={Domain generalization with adversarial feature learning},
  author={Li, Haoliang and Pan, Sinno Jialin and Wang, Shiqi and Kot, Alex C},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5400--5409},
  year={2018}
}

@inproceedings{liu2021dynamic,
  title={Dynamic Color Transform for Wheat Head Detection},
  author={Liu, Chengxin and Wang, Kewei and Lu, Hao and Cao, Zhiguo},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={1278--1283},
  year={2021}
}

@inproceedings{liu2020towards,
  title={Towards domain generalization in underwater object detection},
  author={Liu, Hong and Song, Pinhao and Ding, Runwei},
  booktitle={2020 IEEE International Conference on Image Processing (ICIP)},
  pages={1971--1975},
  year={2020},
  organization={IEEE}
}

@article{everingham2010pascal,
  title={The {P}ascal visual object classes ({VOC}) challenge},
  author={Everingham, Mark and Van Gool, Luc and Williams, Christopher KI and Winn, John and Zisserman, Andrew},
  journal={International Journal of Computer Vision},
  volume={88},
  number={2},
  pages={303--338},
  year={2010},
  publisher={Springer}
}

@article{david2021globalarxiv,
  title={Global wheat head dataset 2021: more diversity to improve the benchmarking of wheat head localization methods},
  author={David, Etienne and Serouart, Mario and Smith, Daniel and Madec, Simon and Velumani, Kaaviya and Liu, Shouyang and Wang, Xu and Espinosa, Francisco Pinto and Shafiee, Shahameh and Tahir, Izzat SA and others},
  journal={arXiv preprint arXiv:2105.07660},
  year={2021}
}

@dataset{david2021dataset,
  author       = {David, Etienne},
  title        = {Global Wheat Head Dataset 2021},
  month        = jul,
  year         = 2021,
  publisher    = {Zenodo},
  version      = {1.0},
  doi          = {10.5281/zenodo.5092309},
  url          = {https://doi.org/10.5281/zenodo.5092309}
}


@inproceedings{li2022learning,
  title={Learning multiple dense prediction tasks from partially annotated data},
  author={Li, Wei-Hong and Liu, Xialei and Bilen, Hakan},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={18879--18889},
  year={2022}
}

@article{ullah2023ssmd,
  title={SSMD-UNet: semi-supervised multi-task decoders network for diabetic retinopathy segmentation},
  author={Ullah, Zahid and Usman, Muhammad and Latif, Siddique and Khan, Asifullah and Gwak, Jeonghwan},
  journal={Scientific Reports},
  volume={13},
  number={1},
  pages={9087},
  year={2023},
}

@article{ganin2016domain,
  title={Domain-adversarial training of neural networks},
  author={Ganin, Yaroslav and Ustinova, Evgeniya and Ajakan, Hana and Germain, Pascal and Larochelle, Hugo and Laviolette, Fran{\c{c}}ois and Marchand, Mario and Lempitsky, Victor},
  journal={The journal of machine learning research},
  volume={17},
  number={1},
  pages={2096--2030},
  year={2016},
  publisher={JMLR. org}
}


@inproceedings{lin2014microsoft,
  title={Microsoft {COCO}: Common objects in context},
  author={Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Doll{\'a}r, Piotr and Zitnick, C Lawrence},
  booktitle={European Conference on Computer Vision},
  pages={740--755},
  year={2014},
  organization={Springer}
}

@inproceedings{yue2019domain,
  title={Domain randomization and pyramid consistency: Simulation-to-real generalization without accessing target domain data},
  author={Yue, Xiangyu and Zhang, Yang and Zhao, Sicheng and Sangiovanni-Vincentelli, Alberto and Keutzer, Kurt and Gong, Boqing},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={2100--2110},
  year={2019}
}

@article{li2020domain,
  title={Domain generalization for medical imaging classification with linear-dependency regularization},
  author={H.~Li and Y.~Wang and R.~Wan and S.~Wang and T-Q.~Li and A.~Kot},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={3118--3129},
  year={2020}
}

@inproceedings{mahajan2021domain,
  title={Domain generalization using causal matching},
  author={D.~Mahajan and S.~Tople and A.~Sharma},
  booktitle={Proceedings of ICML},
  pages={7313--7324},
  year={2021}
}

@article{ghifary2016scatter,
  title={Scatter component analysis: A unified framework for domain adaptation and domain generalization},
  author={M.~Ghifary and D.~Balduzzi and W.B.~Kleijn and M.~Zhang},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={39},
  number={7},
  pages={1414--1430},
  year={2016}
}

@inproceedings{lin2021domain,
  title={Domain-invariant disentangled network for generalizable object detection},
  author={Lin, Chuang and Yuan, Zehuan and Zhao, Sicheng and Sun, Peize and Wang, Changhu and Cai, Jianfei},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={8771--8780},
  year={2021}
}


@inproceedings{li2019episodic,
  title={Episodic training for domain generalization},
  author={Li, Da and Zhang, Jianshu and Yang, Yongxin and Liu, Cong and Song, Yi-Zhe and Hospedales, Timothy M},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={1446--1455},
  year={2019}
}

@article{chen2023achieving,
author = {Chen, Yang and Song, Pinhao and Liu, Hong and Dai, Linhui and Zhang, Xiaochuan and Ding, Runwei and Li, Shengquan},
title = {Achieving Domain Generalization for Underwater Object Detection by Domain Mixup and Contrastive Learning},
year = {2023},
issue_date = {Apr 2023},
publisher = {Elsevier Science Publishers B. V.},
volume = {528},
number = {C},
doi = {10.1016/j.neucom.2023.01.053},
journal = {Neurocomput.},
month = {apr},
pages = {20–34},
}

@article{redmon2018yolov3,
  title={Yolov3: An incremental improvement},
  author={Redmon, Joseph and Farhadi, Ali},
  journal={arXiv preprint arXiv:1804.02767},
  year={2018}
}


@inproceedings{hu2020domain,
  title={Domain generalization via multidomain discriminant analysis},
  author={Hu, Shoubo and Zhang, Kun and Chen, Zhitang and Chan, Laiwan},
  booktitle={Uncertainty in Artificial Intelligence},
  pages={292--302},
  year={2020},
  organization={PMLR}
}



@inproceedings{girshick2014rich,
  title={Rich feature hierarchies for accurate object detection and semantic segmentation},
  author={Girshick, Ross and Donahue, Jeff and Darrell, Trevor and Malik, Jitendra},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={580--587},
  year={2014}
}

@inproceedings{girshick2015fast,
  title={Fast {R-CNN}},
  author={Girshick, Ross},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={1440--1448},
  year={2015}
}

@inproceedings{redmon2016you,
  title={You only look once: Unified, real-time object detection},
  author={Redmon, Joseph and Divvala, Santosh and Girshick, Ross and Farhadi, Ali},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={779--788},
  year={2016}
}

@misc{jocher2020yolov5,
  author       = {Glenn Jocher and Alex Stoken and Jirka Borovec and NanoCode012 and ChristopherSTAN and Liu Changyu and Laughing and tkianai and Adam Hogan and lorenzomammana and
                  yxNONG and AlexWang1900 and
                  Laurentiu Diaconu and
                  Marc and wanghaoyang0106 and ml5ah and Doug and Francisco Ingham and Frederik and
                  Guilhen and Hatovix and
                  Jake Poznanski and    Jiacong Fang and
                  Lijun Yu and changyu98 and Mingyu Wang and Naman Gupta and
                  Osama Akhtar and      PetrDvoracek and
                  Prashant Rai}, 
  title        = {{ultralytics/yolov5: v3.1 - Bug Fixes and Performance Improvements}},
  month        = oct,
  year         = 2020,
  version      = {v3.1}
}

@article{foggy,
  author = {Sakaridis, Christos and Dai, Dengxin and Van Gool, Luc},
  title = {Semantic Foggy Scene Understanding with Synthetic Data},
  journal = {International Journal of Computer Vision},
  year = {2018},
  month = {Sep},
  volume = {126},
  number = {9},
  pages = {973--992}
}

 @InProceedings{rainy_cityscapes,
author = {Hu, Xiaowei and Fu, Chi-Wing and Zhu, Lei and Heng, Pheng-Ann},
title = {Depth-Attentional Features for Single-Image Rain Removal},
booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2019}
}

@inproceedings{bdd100k,
  title={Bdd100k: A diverse driving dataset for heterogeneous multitask learning},
  author={Yu, Fisher and Chen, Haofeng and Wang, Xin and Xian, Wenqi and Chen, Yingying and Liu, Fangchen and Madhavan, Vashisht and Darrell, Trevor},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={2636--2645},
  year={2020}
}

@inproceedings{sim10k,
  title={Driving in the Matrix: Can virtual worlds replace human-generated annotations for real world tasks?},
  author={Johnson-Roberson, Matthew and Barto, Charles and Mehta, Rounak and Sridhar, Sharath Nittur and Rosaen, Karl and Vasudevan, Ram},
  booktitle={2017 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={746--753},
  year={2017},
  organization={IEEE}
}

@inproceedings{tan2020efficientdet,
  title={Efficientdet: Scalable and efficient object detection},
  author={Tan, Mingxing and Pang, Ruoming and Le, Quoc V},
  booktitle={Proceedings of the {IEEE/CVF} Conference on Computer Vision and Pattern Recognition},
  pages={10781--10790},
  year={2020}
}

@inproceedings{liu2016ssd,
  title={{SSD}: Single shot multibox detector},
  author={Liu, Wei and Anguelov, Dragomir and Erhan, Dumitru and Szegedy, Christian and Reed, Scott and Fu, Cheng-Yang and Berg, Alexander C},
  booktitle={European Conference on Computer Vision},
  pages={21--37},
  year={2016},
  organization={Springer}
}

@inproceedings{lin2017feature,
  title={Feature pyramid networks for object detection},
  author={Lin, Tsung-Yi and Doll{\'a}r, Piotr and Girshick, Ross and He, Kaiming and Hariharan, Bharath and Belongie, Serge},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2117--2125},
  year={2017}
}

@inproceedings{jifeng2016rfcn,
 author = {Dai, Jifeng and Li, Yi and He, Kaiming and Sun, Jian},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {D. Lee and M. Sugiyama and U. Luxburg and I. Guyon and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {{R-FCN}: Object Detection via Region-based Fully Convolutional Networks},
 volume = {29},
 year = {2016}
}

@inproceedings{recht2019imagenet,
  title={Do imagenet classifiers generalize to imagenet?},
  author={Recht, Benjamin and Roelofs, Rebecca and Schmidt, Ludwig and Shankar, Vaishaal},
  booktitle={International Conference on Machine Learning},
  pages={5389--5400},
  year={2019},
  organization={PMLR}
}

@inproceedings{seemakurthy2023aaai,
  title={Domain Generalised {Faster} {R-CNN}},
  author={Seemakurthy, Karthik and Fox, Charles and Aptoula, Erchan and Bosilj, Petra},
  year={2023},
  booktitle={Thirty-Seventh AAAI Conference on Artificial Intelligence},
}

@article{bosilj2020transfer,
  title={Transfer learning between crop types for semantic segmentation of crops versus weeds in precision agriculture},
  author={Bosilj, Petra and Aptoula, Erchan and Duckett, Tom and Cielniak, Grzegorz},
  journal={Journal of Field Robotics},
  volume={37},
  number={1},
  pages={7--19},
  year={2020},
  publisher={Wiley Online Library}
}


@inproceedings{wang2019panet,
  title={Panet: Few-shot image semantic segmentation with prototype alignment},
  author={Wang, Kaixin and Liew, Jun Hao and Zou, Yingtian and Zhou, Daquan and Feng, Jiashi},
  booktitle={proceedings of the IEEE/CVF international conference on computer vision},
  pages={9197--9206},
  year={2019}
}

@inproceedings{noroozi2016unsupervised,
  title={Unsupervised learning of visual representations by solving jigsaw puzzles},
  author={Noroozi, Mehdi and Favaro, Paolo},
  booktitle={European conference on computer vision},
  pages={69--84},
  year={2016},
  organization={Springer}
}

@article{hindel2023inod,
  title={INoD: Injected Noise Discriminator for Self-Supervised Representation Learning in Agricultural Fields},
  author={Hindel, Julia and Gosala, Nikhil and Bregler, Kevin and Valada, Abhinav},
  journal={arXiv preprint arXiv:2303.18101},
  year={2023}
}

@article{ilteralp2021deep,
  title={A deep multitask semisupervised learning approach for chlorophyll-a retrieval from remote sensing images},
  author={Ilteralp, Melike and Ariman, Sema and Aptoula, Erchan},
  journal={Remote Sensing},
  volume={14},
  number={1},
  pages={18},
  year={2021},
  publisher={MDPI}
}


@inproceedings{yang2016deep,
  title={Deep Multi-task Representation Learning: A Tensor Factorisation Approach},
  author={Yang, Yongxin and Hospedales, Timothy M},
  booktitle={International Conference on Learning Representations},
  year={2016}
}


@inproceedings{wang2020learning,
  title={Learning from extrinsic and intrinsic supervisions for domain generalization},
  author={Wang, Shujun and Yu, Lequan and Li, Caizi and Fu, Chi-Wing and Heng, Pheng-Ann},
  booktitle={European Conference on Computer Vision},
  pages={159--176},
  year={2020},
  organization={Springer}
}




@article{jing2020self,
  title={Self-supervised visual feature learning with deep neural networks: A survey},
  author={Jing, Longlong and Tian, Yingli},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={43},
  number={11},
  pages={4037--4058},
  year={2020},
  publisher={IEEE}
}



@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={2009 IEEE conference on computer vision and pattern recognition},
  pages={248--255},
  year={2009},
  organization={Ieee}
}


@article{pan2010survey,
  title={A survey on transfer learning},
  author={Pan, Sinno Jialin and Yang, Qiang},
  journal={IEEE Transactions on knowledge and data engineering},
  volume={22},
  number={10},
  pages={1345--1359},
  year={2010},
  publisher={IEEE}
}


@inproceedings{seemakurthy2023icra,
  title={Domain Generalised Fully Convolutional One Stage Detection},
  author={Seemakurthy, Karthik and Bosilj, Petra and Aptoula, Erchan and Fox, Charles},
  year={2023},
  publisher={IEEE},
  booktitle={International Conference on Robotics and Automation (ICRA)}
}


@inproceedings{tian2019fcos,
  title={Fcos: Fully convolutional one-stage object detection},
  author={Tian, Zhi and Shen, Chunhua and Chen, Hao and He, Tong},
  booktitle={Proceedings of the IEEE/CVF international conference on computer vision},
  pages={9627--9636},
  year={2019}
}


@article{hendrycks2019benchmarking,
  title={Benchmarking neural network robustness to common corruptions and perturbations},
  author={Hendrycks, Dan and Dietterich, Thomas},
  journal={arXiv preprint arXiv:1903.12261},
  year={2019}
}

@inproceedings{li2020deep,
  title={Deep domain adaptive object detection: A survey},
  author={Li, Wanyi and Li, Fuyu and Luo, Yongkang and Wang, Peng and others},
  booktitle={2020 IEEE Symposium Series on Computational Intelligence (SSCI)},
  pages={1808--1813},
  year={2020},
  organization={IEEE}
}

@inproceedings{sindagi2020prior,
  title={Prior-based domain adaptive object detection for hazy and rainy conditions},
  author={Sindagi, Vishwanath A and Oza, Poojan and Yasarla, Rajeev and Patel, Vishal M},
  booktitle={European Conference on Computer Vision},
  pages={763--780},
  year={2020},
  organization={Springer}
}

@article{rosenfeld2020risks,
  title={The risks of invariant risk minimization},
  author={Rosenfeld, Elan and Ravikumar, Pradeep and Risteski, Andrej},
  journal={arXiv preprint arXiv:2010.05761},
  year={2020}
}
@article{arjovsky2019invariant,
  title={Invariant risk minimization},
  author={Arjovsky, Martin and Bottou, L{\'e}on and Gulrajani, Ishaan and Lopez-Paz, David},
  journal={arXiv preprint arXiv:1907.02893},
  year={2019}
}

@inproceedings{he2019multi,
  title={Multi-adversarial {Faster R-CNN} for unrestricted object detection},
  author={He, Zhenwei and Zhang, Lei},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={6668--6677},
  year={2019}
}

@misc{cvpr2018_pytorch,
  author = {Jianwei Yang, sumiya-NJU},
  howpublished = "\url{https://github.com/tiancity-NJU/da-faster-rcnn-PyTorch}",
  year = {2008}, 
  note = "[Online; accessed 19-July-2008]"
}

@inproceedings{saito2019strong,
  title={Strong-weak distribution alignment for adaptive object detection},
  author={Saito, Kuniaki and Ushiku, Yoshitaka and Harada, Tatsuya and Saenko, Kate},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={6956--6965},
  year={2019}
}
@inproceedings{xu2020exploring,
  title={Exploring categorical regularization for domain adaptive object detection},
  author={Xu, Chang-Dong and Zhao, Xing-Ran and Jin, Xin and Wei, Xiu-Shen},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11724--11733},
  year={2020}
}

@inproceedings{zhu2019adapting,
  title={Adapting object detectors via selective cross-domain alignment},
  author={Zhu, Xinge and Pang, Jiangmiao and Yang, Ceyuan and Shi, Jianping and Lin, Dahua},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={687--696},
  year={2019}
}

@inproceedings{hsu2020progressive,
  title={Progressive domain adaptation for object detection},
  author={Hsu, Han-Kai and Yao, Chun-Han and Tsai, Yi-Hsuan and Hung, Wei-Chih and Tseng, Hung-Yu and Singh, Maneesh and Yang, Ming-Hsuan},
  booktitle={Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages={749--757},
  year={2020}
}

@inproceedings{rodriguez2019domain,
  title={Domain adaptation for object detection via style consistency},
  author={Rodriguez, Adrian Lopez and Mikolajczyk, Krystian},
  booktitle={Proceedings BMVC},
  year={2019}
}

@inproceedings{khodabandeh2019robust,
  title={A robust learning approach to domain adaptive object detection},
  author={Khodabandeh, Mehran and Vahdat, Arash and Ranjbar, Mani and Macready, William G},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={480--490},
  year={2019}
}

@inproceedings{roychowdhury2019automatic,
  title={Automatic adaptation of object detectors to new domains using self-training},
  author={RoyChowdhury, Aruni and Chakrabarty, Prithvijit and Singh, Ashish and Jin, SouYoung and Jiang, Huaizu and Cao, Liangliang and Learned-Miller, Erik},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={780--790},
  year={2019}
}

@incollection{middleton1957vision,
  title={Vision through the atmosphere},
  author={Middleton, William Edgar Knowles},
  booktitle={Geophysik II/Geophysics II},
  pages={254--287},
  year={1957},
  publisher={Springer}
}

@inproceedings{yao2021multi,
  title={Multi-Source Domain Adaptation for Object Detection},
  author={Yao, Xingxu and Zhao, Sicheng and Xu, Pengfei and Yang, Jufeng},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={3273--3282},
  year={2021}
}

@article{goodfellow2014generative,
  title={Generative adversarial networks},
  author={Goodfellow, Ian J and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1406.2661},
  year={2014}
}

@inproceedings{dalal2005histograms,
  title={Histograms of oriented gradients for human detection},
  author={Dalal, Navneet and Triggs, Bill},
  booktitle={2005 IEEE Computer Society Conference on Computer Vision and Pattern Recognition (CVPR'05)},
  volume={1},
  pages={886--893},
  year={2005},
  organization={Ieee}
}

@article{felzenszwalb2009object,
  title={Object detection with discriminatively trained part-based models},
  author={Felzenszwalb, Pedro F and Girshick, Ross B and McAllester, David and Ramanan, Deva},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={32},
  number={9},
  pages={1627--1645},
  year={2009}
}

@inproceedings{viola2001rapid,
  title={Rapid object detection using a boosted cascade of simple features},
  author={Viola, Paul and Jones, Michael},
  booktitle={Proceedings of the 2001 IEEE Computer Society Conference on Computer Vision and Pattern Recognition. CVPR 2001},
  volume={1},
  pages={I--I},
  year={2001},
  organization={Ieee}
}

@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={Ieee}
}

@article{blanchard2011generalizing,
  title={Generalizing from several related classification tasks to a new unlabeled sample},
  author={Blanchard, Gilles and Lee, Gyemin and Scott, Clayton},
  journal={Advances in neural information processing systems},
  volume={24},
  pages={2178--2186},
  year={2011}
}

@inproceedings{zhou2020learning,
  title={Learning to generate novel domains for domain generalization},
  author={Zhou, Kaiyang and Yang, Yongxin and Hospedales, Timothy and Xiang, Tao},
  booktitle={Computer Vision--ECCV 2020: 16th European Conference, Glasgow, UK, August 23--28, 2020, Proceedings, Part XVI 16},
  pages={561--578},
  year={2020},
  organization={Springer}
}


@article{zhou2021domain,
  title={Domain generalization: A survey},
  author={Zhou, Kaiyang and Liu, Ziwei and Qiao, Yu and Xiang, Tao and Loy, Chen Change},
  journal={arXiv preprint arXiv:2103.02503},
  year={2021}
}

@article{krizhevsky2012imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  journal={Advances in neural information processing systems},
  volume={25},
  pages={1097--1105},
  year={2012}
}


